Analyzing Smart Contracts: From EVM to a sound Control-Flow Graph

The EVM language is a simple stack-based language with words of 256 bits, with one significant difference between the EVM and other virtual machine languages (like Java Bytecode or CLI for .Net programs): the use of the stack for saving the jump addresses instead of having it explicit in the code of the jumping instructions. Static analyzers need the complete control flow graph (CFG) of the EVM program in order to be able to represent all its execution paths. This report addresses the problem of obtaining a precise and complete stack-sensitive CFG by means of a static analysis, cloning the blocks that might be executed using different states of the execution stack. The soundness of the analysis presented is proved.

==> proof1.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%

\section{Proof for Theorem~\ref{theorem:cfganalysis}}

The proof sketch follows the next steps:

\begin{enumerate}
\item We first define an \EVM operational semantics that describes how
  \EVM programs handle jump addresses on the stack.

\item Then we define an \EVM collecting semantics for the operational
  semantics. Such collecting semantics gathers all transitions that
  can be produced by the execution of a program $P$;
\item We continue by defining the jumps-to property as a property of
  this collecting semantics; and
\item Then we prove a lemma that states that the least solution of the
  set of constraints generated as described in
  Definition~\ref{def:jumpeq} is a safe approximation of the \EVM
  collecting semantics w.r.t. the jumps-to property.
\item Finally, we rewrite Theorem~\ref{theorem:cfganalysis} in terms
  of the operational semantics and prove it.
\end{enumerate}

\input{semantics-al}

Figure~\ref{fig:jumpsemantics} shows the semantics of some
instructions involved in the computation of the values stored in the
stack for handling jumps.  The state of the program $S$ is a tuple
$\tuple{pc, \tuple{n,\sigma}}$ where $pc$ is the value of the program
counter with the index of the next instruction to be executed, and
$\tuple{n,\sigma}$ is a \emph{stack state} as defined in
Section~\ref{sec:from-evm-to-cfg}.
%
%
Interesting rules are the ones that deal with jump destination addresses
on the stack:  Rule \textsc{(4)} adds a new address on the stack, and
Rules  \textsc{(6)} and \textsc{(8-10)} copy or exchange existing
addresses on top of the stack, respectively. 
%
Rules \textsc{(1)} to \textsc{(3)} perform a jump in the program and
therefore consume the address placed on top of the stack, plus an
additional word in the case of \code{JUMPI}.  If the
instructions considered in this simplified semantics do not handle 
jump addresses, the corresponding rules just remove some values from
the stack in the program state $S$ (Rules \textsc{(5)}, \textsc{(7)}
and \textsc{(11)}).
%
The remaining \EVM instructions not explicitely considered in this
simplified semantics are generically represented by Rule \textsc{(12)}
with $b_{pc}^{\delta , \alpha}$, where $\delta$ is the number of items
removed from stack when $b_{pc}$ is executed, and $\alpha$ is the
number of additional items placed on the stack.
%
Complete executions are traces of the form
$S_0 \rrderivproof S_1 \rrderivproof \dots \rrderivproof S_n$ where $S_0 \equiv
\tuple{0, \tuple{0,\sigma_{\emptyset}}}$ is the initial
state, $\sigma_{\empty}$ is the empty mapping, and $S_n$ corresponds
to the last state.  There are no infinite traces, as any transaction
that executes \EVM code has a finite gas limit and every instruction
executed consumes some amount of gas.  When the gas limit is exceeded,
an out-of-gas exception occurs and the program halts immediately.



% \begin{definition}

% Given an \EVM program $ P \equiv b_0, ..., b_p$ and the constraint equation system
% defined in Section~\ref{eq:equation_system} with constraint variables
% $\eqn_0,\dots, \eqn_p$, we will use $\eqn_i^m$ to refer to the
% constraint variable $\eqn_i$ after evaluating in iteration $m$. We
% will denote with
% $\eqn_i^0$ the value of $\eqn_i$ after initializing it.

% \end{definition}

%%%%%%%%%%%%%%%%%%%%
\newcommand{\colsemp}{\ensuremath{\mathcal{C}_P}}
\begin{definition}[\EVM collecting semantics]
  Given an \EVM program $P$, the \EVM collecting semantics operator
  $\colsemp$ is defined as follows:
\[
\colsemp (X) = \set{\tuple{S,S'} ~|~ \tuple{\_,S} \in X \wedge S \rrderivproof S'}
\]
The \EVM semantics is defined as $\xi_P = \bigcup_{n>0}
\colsemp^n(X_0)$,  where $X_0 \equiv \set{\tuple{0,\tuple{0,\sigma_{\emptyset}}}}$ is the initial configuration.

\end{definition}

\begin{definition}[jumps-to property]
  Let $P$ be an IR program, $\xi_P = \bigcup_{n>0} \colsemp^n(X_0)$,
  and $b$ an instruction at program point $pc$, then we say
  that $\xi_P \vDash_{pc} T$ ~if~
  $T = \set{ \tuple{n,\sigma} ~|~ \tuple{S,S'}\in\xi_P \wedge
    \tuple{n,\sigma} \in S'}$.

\end{definition}

The following lemma states that the least solution of the constraint
equation system defined in Definition~\ref{eq:equation_system}
is a safe approximation of $\xi_P$:

\begin{lemma}[soundness]
\label{lem:soundness}
  Let $P \equiv b_0,\dots, b_p$ be a program, $pc$ a program point and
  $\eqn_{0},\dots, \eqn_{p}$ the least solution of the constraints
  equation system as defined in Section~\ref{sec:from-evm-to-cfg}.
  The following holds:

  \begin{center}
    If $\xi_P \vDash_{pc} T$, then for all $\tuple{n,\sigma}\in
  T$, exists $s \in dom(\eqn_{pc})$ such that $\tuple{n,\sigma} \in\eqn_{pc}(s)$.
  \end{center}
\end{lemma}

\begin{proof}
We use $\eqn_{pc}^m$ to refer to the value obtained for $\eqn_{pc}$
after $m$ iterations of the algorithm for solving the equation system
depicted in Section~\ref{sec:from-evm-to-cfg}.
%
We say that $\eqn_{pc}$
\emph{covers} $\tuple{n,\sigma}$ in $\colsemp^m(X_0)$ at program point
$pc$ when this lemma holds for the result of computing
$\colsemp^m(X_0)$.
%
In order to prove this lemma, we can reason by induction on
the value of $m$, the length of the traces $S_0 \rrderivproof^m S_m$ considered
in $\colsemp^m(X_0)$.

\textbf{Case base}: if $m = 0$,
$S_0 = \tuple{0,\tuple{0, \sigma_{\emptyset}}}$ and the Lemma
trivially holds as 
$\tuple{0, \sigma_{\emptyset}} \in \eqn_0^0(\tuple{0,
  \sigma_{\emptyset}})$.

\textbf{Induction Hypothesis}: we assume Lemma~\ref{lem:soundness} holds for all
traces of length $m \geq 0$.

\textbf{Inductive Case}: Let us consider traces of length $m + 1$,
which are of the form $S_0 \rrderivproof^m S_m \rrderivproof S_{m+1}$. $S_m$ is
a program state of the form $S_m = \tuple{pc, \tuple{n, \sigma}}$.  We
can apply the induction hypothesis to $S_m$: there exists some
$s\in dom(\eqn_{pc}^m)$ such that
$ \tuple{n, \sigma} \in \eqn_{pc}^{m}(s) $. For extending the Lemma, we
reason for all possible rules in the simplified \EVM semantics
(Fig.~\ref{EVM_semantics}) we may apply from $S_m$ to $S_{m+1}$:

\begin{itemize}
\item{Rule (1)}: After executing a \code{JUMP} instruction $S_{m+1}$
  is of the form
  $\tuple{\sigma(s_{n-1}), \tuple{n-1,
      \sigma\backslash[s_{n-1}]}}$.
  In iteration $m+1$, the following set of equations corresponding to
  $b_{pc}$ is evaluated:
%
\[ 
\begin{array}{rcll}
\eqn_{\sigma(s_{n-1})} & \sqsupseteq & \textit{idmap}(\lambda(b_{pc},
\tuple{n', \sigma'})) & \text{~~~for all~}s'\in dom(\eqn_{pc}), \tuple{n', \sigma'} \in \eqn_{pc}(s')
\end{array}
\]
%
where
$\textit{idmap}(\lambda(b_{pc}, \langle n', \sigma'
\rangle)) = \pi_{\bot}[ \tuple{n'-1,\sigma'\backslash[s_{n-1}]} \mapsto
\set{\tuple{n'-1,\sigma'\backslash[s_{n-1}]}}]$ (Case (4) in Fig.~\ref{fig:transfer}).
%
The induction hypothesis guarantees that there exists some $s'' \in
\eqn_{pc}^{m}$ such that 
$ \tuple{n, \sigma} \in \eqn_{pc}^{m}(s'') $, where $S_m = \tuple{pc,
  \tuple{n, \sigma}}$.  Therefore, at
Iteration $m+1$, the following must hold:
%
\[ 
\eqn_{\sigma(s_{n-1})}^{m+1} \sqsupseteq
\pi_{\bot}[ \tuple{n-1,\sigma\backslash[s_{n-1}]} \mapsto \set{\tuple{n-1,\sigma\backslash[s_{n-1}]}}]
\]
%
so $\tuple{n-1,\sigma\backslash[s_{n-1}]} \in
\eqn_{\sigma(s_{n-1})}^{m+1}(\tuple{n-1,\sigma\backslash[s_{n-1}]})$
and thus Lemma~\ref{lem:soundness} holds.

\item{Rules (2) and (3)}: After executing a \code{JUMPI} instruction,
  $S_{m+1}$ is either
  $\tuple{\sigma(s_{n-1}), \tuple{n-2, \sigma\backslash[s_{n-1},
      s_{n-2}]}}$
  or $\tuple{pc+size(b_{pc}), \tuple{n-2, \sigma\backslash[s_{n-1}, s_{n-2}]}}$,
  respectively.  In any of those cases the following sets of equations
  are evaluated:
%
\[
\begin{array}{rcll}
\eqn_{\sigma(s_{n-2})} & \sqsupseteq & \textit{idmap}(\lambda(\text{\code{JUMPI}},
\langle n', \sigma' \rangle)) & \text{~~~for all~} s'\in dom(\eqn_{pc}), \tuple{n', \sigma'} \in \eqn_{pc}(s')
\\
\eqn_{pc+1} & \sqsupseteq & \textit{idmap}(\lambda(\text{\code{JUMPI}},
\langle n', \sigma' \rangle)) & \text{~~~for all~} s'\in dom(\eqn_{pc}), \tuple{n', \sigma'} \in \eqn_{pc}(s')
\end{array}
\]
%
where
$\textit{idmap}(\lambda(b_{pc}, \langle n', \sigma' \rangle)) =
\pi_{\bot}[ \tuple{n'-2,\sigma'\backslash[s_{n-1},s_{n-2}]} \mapsto
\set{\tuple{n'-2,\sigma'\backslash[s_{n-1},s_{n-2}]}}]$
(Case (4) of the definition of the update function $\lambda$ in
Fig.~\ref{fig:transfer}). 
%
As in the previous case, the induction hypothesis guarantees that at
Iteration $m$ there exists $s'' \in
\eqn_{pc}^{m}$ such that 
$ \tuple{n, \sigma} \in \eqn_{pc}^{m}(s'') $. Therefore, in 
Iteration $m+1$, the following must hold:
%
\[ 
\begin{array}{rcl}
\eqn_{\sigma(s_{n-1})}^{m+1} & \sqsupseteq &
\pi_{\bot}[ \tuple{n-2,\sigma\backslash[s_{n-1},s_{n-2}]} \mapsto \set{\tuple{n-2,\sigma\backslash[s_{n-1},s_{n-2}]}}]
\\
\eqn_{pc+1}^{m+1} & \sqsupseteq &
\pi_{\bot}[ \tuple{n-2,\sigma\backslash[s_{n-1},s_{n-2}]} \mapsto \set{\tuple{n-2,\sigma\backslash[s_{n-1},s_{n-2}]}}]
\end{array}
\]
%
and thus Lemma~\ref{lem:soundness} holds for these cases as well.


\item{Rules (4) - (12)}: We will first consider the
  case in which any of these rules corresponds to an \EVM instruction
  followed by an instruction different from \code{JUMPDEST}.  All
  rules are similar, as they all use the set of equations generated by
  Case (4) in Definition~\ref{def:jumpeq}.  We will see Rule (4) in detail.

After executing a
  $\text{\code{PUSH}}x~v$ instruction, $S_{m+1}$ is
  $\tuple{pc+size(b_{pc}), \tuple{n+1, \sigma[s_{n} \mapsto
      \set{v}]}}$.  We have to prove that exists some $s
  \in dom(\eqn_{pc+size(b_{pc})})$ such that $\tuple{n+1, \sigma[s_{n} \mapsto
      \set{v}]} \in \eqn_{pc+size(b_{pc})}(s)$.
%
  The following set of equations is evaluated:
%
\begin{equation}
\label{eq:rule4-1}
\begin{array}{rcll}
\eqn_{pc+size(b_{pc})} & \sqsupseteq & \tau(\text{\code{PUSH}}x,
\eqn_{pc})
\end{array}
\end{equation}
%
By Definition~\ref{def:transfer}, $\tau (\text{\code{PUSH}}x,
\eqn_{pc}) = \pi'$, where
$\forall s' \in dom(\pi), \pi'(s') = \lambda(\text{\code{PUSH}}x,
\eqn_{pc}(s'))$.   By the case (1) of the definition of the update
function $\lambda$, we have that:
%
\begin{equation}
  \label{eq:rule4-2}
\forall \tuple{n'', \sigma''} \in dom(\eqn_{pc}), \pi'(\tuple{n'',
  \sigma''}) = \tuple{n''+1, \sigma''[s_n \mapsto
  \set{v}]} 
\end{equation}


By the induction hypothesis, at Iteration $m$ there exists some $s \in
dom(\eqn^m_{pc})$ such that $\tuple{n,\sigma} \in \eqn^m_{pc}(s)$.
Therefore, by~\ref{eq:rule4-1} and~\ref{eq:rule4-2}, at Iteration
$m+1$ we have that the following holds:
%
\[
 s \in dom(\eqn^{m+1}_{pc+size(b_{pc})}) ~\text{and}~ 
 \tuple{n+1, \sigma[s_{n} \mapsto
   \set{v}]} \in \eqn_{pc+size(b_{pc})}(s)
\]
%
and thus Lemma~\ref{lem:soundness} holds for Rule (4).


\item{Rules (4) - (12)}, followed by a \code{JUMPDEST} instruction.
%
After executing any of these instructions, $S_{m+1}$ is
  $\tuple{pc+size(b_{pc}), \tuple{n''', \sigma'''}}$, where
  $\tuple{n''', \sigma'''}$ is obtained according to the rule from
  Figure~\ref{fig:jumpsemantics}.  
  We have to prove that exists some $s
  \in dom(\eqn_{pc+size(b_{pc})})$ such that $\tuple{n''', \sigma'''}
  \in \eqn_{pc+size(b_{pc})}(s)$. 
%
  The following set of equations is evaluated:
%
\begin{equation}
\label{eq:rule4-3}
\begin{array}{rcll}
\eqn_{pc+size(b_{pc})} & \sqsupseteq & \textit{idmap}(\lambda(b_{pc},
\langle n', \sigma' \rangle)) & \text{~~~for all~} s'\in dom(\eqn_{pc}), \tuple{n', \sigma'} \in \eqn_{pc}(s')
\end{array}
\end{equation}
%
where
$\textit{idmap}(\lambda(b_{pc}, \langle n', \sigma' \rangle)) =
\pi_{\bot}[ \tuple{n'',\sigma'']} \mapsto
\set{\tuple{n'',\sigma''}}]$, where $n''$ and $\sigma`$ are obtained
according to the cases of the updating function detailed in
Figure~\ref{fig:transfer}.  We can see that
$\set{\tuple{n'',\sigma''}}]$ match the modification made to the state
$S_{m+1}$ by the corresponding rule of the semantics.  Therefore, at Iteration
there exists an $s = \set{\tuple{n'',\sigma''}}]$ such that
$\set{\tuple{n'',\sigma''}}] \in \eqn_{pc+size(b_{pc})}^{m+1}$, and
Lemma~\ref{lem:soundness} also holds.
\end{itemize}

When the algorithm stops Lemma~\ref{lem:soundness} holds, as for any
$pc$ $\eqn_{pc}^{m+1} \sqsupseteq \eqn_{pc}^{m}$ for each iteration of
the algorithm for solving the equations system of
Section~\ref{sec:from-evm-to-cfg}.
\end{proof}

Now we rewrite Theorem~\ref{theorem:cfganalysis} in terms of the
operational semantics of Figure~\ref{fig:jumpsemantics}. This
rewriting actually is stronger than Theorem~\ref{theorem:cfganalysis},
as guarantees the correctness of the stack states obtained from the
jumps equations system at any step of the execution.

\begin{theorem}[Soundness]
  \label{theorem:appendix}
  Let $P \equiv b_0,\dots,b_p$ be a program,
  $S_0 = \tuple{0, \tuple{0, \sigma_{\emptyset}}}$ the initial
  program state, and $\eqn_1,\dots,\eqn_n$ the solution of the jumps
  equations system of $P$. Then for any trace $S_0 \rrderiv^{*} S_m$, where
  $S_m = \tuple{pc, \tuple{n, \sigma}} $, there exists $s \in
  dom(\eqn_{pc})$ such that $ \tuple{n, \sigma} \in \eqn_{pc}(s) $.
\end{theorem}

\begin{proof}
  Straightforward from Lemma~\ref{lem:soundness}, as the \EVM
  collecting semantics takes into account all possible traces of the
  operational semantics.
\end{proof}


==> proof2.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%

\mycomment{
\section{Proof Sketch for Theorem~\ref{theorem:cfganalysis2}}





}


==> semantics.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%

\subsection{Semantics of the Annotated Rule-Based Representation}
\label{sec:semantics}


\begin{figure}[t]\centering
%  \begin{tabular}{|x{0.7cm}x{10cm}|}
  \begin{tabular}{|cc|}
\hline
\textsc{(1)} & 
      \rrrulewide{b \equiv s_i = expr, s_i\in dom(\semstack), eval(expr,\semstack,\semlocal,\semstorage) = v}
      {
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}
        \rrderiv
\semstatetuple{\tuple{p, bs, \semstack[s_i\mapsto v]}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}}

\ruleskip

\textsc{(2)} & 
      \rrrulewide{b \equiv s_i = \yellowblockchain(bc), s_i\in dom(st), bc\in \blockchainvars, \semblockchain(bc) = v}
      {
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}
        \rrderiv
\semstatetuple{\tuple{p, b \cdot bs, \semstack[s_i\mapsto v]}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}}

\ruleskip

\textsc{(3)} & 
      \rrrulewide{b \equiv \yellowmemory[s_j] = s_i, s_i\in dom(\semstack),
               s_j\in dom(\semstack), \semstack(s_i) = v, \semstack(s_j) = id}
      {
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}
        \rrderiv
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal[id\mapsto v]}{\semstorage}{\semgasop}{\semgasmem}}

\ruleskip

\textsc{(4)} & 
      \rrrulewide{b \equiv \yellowstorage[s_j] = s_i, s_i\in
               dom(\semstack), s_j\in dom(\semstack), \semstack(s_i) =
               v, \semstack(s_j) = id}
      {
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}
        \rrderiv
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage[id\mapsto v]}{\semgasop}{\semgasmem}}

\ruleskip

\textsc{(5)} & 
      \rrrulewide{b \equiv \text{\code{nop}}(instr), instr \not\in Call, \opcost(instr,\semstack,
               \semstorage) = gas_{o}, \memcost(instr,\semstack) = gas_{m},\\

\semgasop' =
    \semgasop + gas_o, \semgasmem' = \max(\semgasmem,gas_m),
\semgasop' + \semgasmem' \leq \semblockchain(\text{\code{GAS}})}
      {
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}
        \rrderiv %\\
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop'}{\semgasmem'}}

\ruleskip

\textsc{(6)} & 
      \rrrulewide{b \equiv \text{\code{nop}}(instr), instr \in Call, \opcost(instr,\semstack,
               \semstorage) = gas_{o}, \memcost(instr,\semstack) =
                gas_{m},\\
 \extcall(instr,\semstack, \semlocal, \semstorage) = \tuple{\semlocal_{e}, \semstorage_{e}, gas_{e}}, \\
 \semgasop' =
    \semgasop + gas_o + gas_{e}, \semgasmem' = \max(\semgasmem,gas_m),
\semgasop' + \semgasmem' \leq
    \semblockchain(\text{\code{GAS}})}
      {
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}
        \rrderiv %\\
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal_{e}}{\semstorage_{e}}{\semgasop'}{\semgasmem'}}

\ruleskip

% \textsc{(7)} & 
%       \rrrulewide{b \equiv
%         call(q(\sot{q})), ~~
% %        \text{there is a rule~}
%         q(\sot{q}') \Rightarrow
%         bs_q \in RBR, 
%     \semstack_q = \semstack_{\emptyset}, 
%          \forall s_i\in \sot{q}.\semstack_q[s_i \mapsto \semstack(s_i)] }
%       {
% \semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}
%         \rrderiv
% \semstatetuple{\tuple{q, bs_q, \semstack_q}\cdot\tuple{p, bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}}

% \ruleskip

\textsc{(7)} & 
      \rrrulewide{b \equiv
        call(q(\sot{q})), ~~
%        \text{there is a rule~}
        q(\sot{q}') \Rightarrow
        g_q | bs_q \in RBR, \\
    eval(g_q, \semstack) = true, \semstack_q = \semstack_{\emptyset}, 
         \forall s_i\in \sot{q}.\semstack_q[s_i \mapsto \semstack(s_i)] }
      {
\semstatetuple{\tuple{p, b \cdot bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}
        \rrderiv
\semstatetuple{\tuple{q, bs_q, \semstack_q}\cdot\tuple{p, bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}}

\ruleskip

\textsc{(8)} & 
      \rrrulewide{}
      {
\semstatetuple{\tuple{q, \epsilon, \_}\cdot\tuple{p, bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}

        \rrderiv
\semstatetuple{\tuple{p, bs, \semstack}\cdot \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}}

\\ \hline %\ruleskip
    
  \end{tabular}
\secbeg
\caption{Concrete RBR Semantics\label{Summarized_semantics}}
\secbeg\secbeg\secbeg
\end{figure}


Rules in Figure~\ref{Summarized_semantics} define an \emph{operational
  semantics} for the annotated RBR.
%
We use $a\cdot as$ to denote a non-empty sequence of elements, where
$as$ can be the empty sequence, denoted as $\epsilon$.
%
An \emph{activation record} has the form $\tuple{r,bs, \semstack}$,
where $r$ is a rule name, $bs$ is a sequence of instructions in $r$,
if it is not empty is denoted as $b\cdot bs$ where $b$ is the next
instruction to be executed, and $\semstack$ is a mapping of stack
variables to their values $\semstack: \stackvars \mapsto \allvalues$,
where \allvalues\ is the set of all possible values that can be stored
in an \EVM word, i.e.,
$\allvalues = \{ z\in \naturals \cup \{0\} \mid z < 2^{256}\}$.

A \emph{program state} $\semstate$ has the form
$\semstatetuple{\semarecord\cdot
  \semarecords}{\semlocal}{\semstorage}{\semgasop}{\semgasmem}$
where $\semarecord\cdot\semarecords$ is a sequence of activation
records,
%
$\semlocal$ is a mapping of local memory addresses to their values\footnote{Although the
  local memory is byte addressable with instruction \code{MSTORE8},
  for the sake of keeping the semantics simple we
  will only consider the general case of word-addressable \code{MSTORE}.}
$\semlocal: \allvalues \mapsto \allvalues$, $\semstorage$ is a mapping
of storage addresses to their values $\semstorage: \allvalues \mapsto \allvalues$,
$\semblockchain$ is a mapping of blockchain variables
$\semblockchain: \blockchainvars \mapsto \allvalues$,
%
and $\semgasop, \semgasmem \in \naturals \cup \{0\}$ correspond to the
gas consumption accumulated up to the current state of the execution
for instructions execution and memory allocation, respectively.
%
Rule~\textsc{(1)} handles the assignment of an expression to a stack
variable $s_i$.  According to the grammar seen before, this expression
can be a constant, the contents of a memory or storage address, the
contents of a blockchain variable, an arithmetic operation between
stack variables, or some other operations represented by a functor as
for example $xor(s_i,s_j)$. Function
$eval(expr,\semstack,\semlocal,\semstorage)$
% 
%
evaluates the expression using 256-bit arithmetics with respect to the
mappings of stack, memory and storage variables.
%
Rules~\textsc{(2)} to~\textsc{(4)} correspond to assignments of stack
variables to memory or storage elements.
%
Rule~\textsc{(5)} corresponds to the evaluation of a \nop annotation
of any \EVM instruction except external calls, \ie the ones in the set
$Call = \{\text{\code{CALL}}, \text{\code{CALLCODE}},
\text{\code{DELEGATECALL}}, \text{\code{STATICCALL}} \}$.  At this
point the gas consumption $\semgasop, \semgasmem$ in the program state
must be updated with the cost of the corresponding \EVM
instruction. For this purpose, functions
$\opcost(instr,\semstack,\semstorage)$ and $\memcost(instr,\semstack)$
compute the gas consumed by $instr$ as defined in Appendix H
of~\cite{yellow} and will be explained in
Section~\ref{sec:opcode-model} and Section~\ref{sec:memory-model} for
some representative cases. % Given an \EVM instruction $instr$ wrapped
% in $\nop(instr)$, the state of the stack $\semstack$, and the mapping
% of state variables $\semstorage$, the functions $\opcost$ and
% $\memcost$ return the gas consumption of the \EVM instruction
% represented in $instr$, as we will see in
% Section~\ref{sec:concrete-rbr-cost-model}.
% Appendix H.1 of~\cite{yellow}.
%
\code{GAS} is the blockchain variable that contains the amount of
available gas for the current transaction.  We do not consider the
block gas limit in this semantics as it would require taking into
account all transactions executed for building the next blockchain
block.
%
The instructions that correspond to external calls, i.e., those in set
$Call$, are handled separately by Rule~\textsc{(6)}. In this case,
besides the gas consumed by the instruction itself, the gas limit must
also consider the gas consumed by the external contract execution.  In
addition, the external call might change the data stored in memory and
storage (for instance, external contracts might perform callback calls
to the current contract, possibly modifying storage variables),
according to the specification of call instructions in~\cite{yellow}.
This is expressed in the semantics by a call to the function
$\extcall(instr,\semstack,\semlocal,\semstorage)$, that returns a
tuple $\tuple{\semlocal_{e},\semstorage_{e},gas_{e}}$ that contain the
state of the local memory and the storage after executing the external
call, as well as the gas consumed by the executed contract,
respectively.
%
Rule~\textsc{(7)} evaluates a call to a rule in the
RBR.  A fresh activation record is created containing the code of the
called rule, and the argument values are passed to it.
%
Finally, Rule~\textsc{(8)} corresponds to the termination of an
activation record.

\paragraph{Program execution.}
The execution of a smart contract $P$ is initiated in a transaction by
means of a message that includes a function encoded in the input
arguments to be invoked on $P$, as well as other blockchain
information.  Besides, the smart contract is associated to a
persistent storage area on the blockchain that contains the values
assigned so far to its state variables.
%
Therefore, the initial state $\semstate_0$ is of the form
$\tuple{\tuple{\mmcode{block}0,b\cdot bs, \semstack_{\emptyset}},
  \semlocal_{\emptyset},\seminitialstorage,0,0}$, where
\mmcode{block}$0$ is the RBR rule for the first block in the smart
contract, $b\cdot bs$ is the block code, $\semstack_{\emptyset}$ and
$\semlocal_{\emptyset}$ represent the empty mappings for stack
variables and local variables, respectively, and $\seminitialstorage$
contains the current mapping of state variables to their values in the
blockchain. Additionally, $\semblockchain$ contains the current state
of blockchain variables.

A trace is of the form
$t \equiv \semstate_{0} \rrderiv\cdots\rrderiv
\semstate_{i}\rrderiv\cdots\semstate_{n}$.  As we have already
mentioned, there are no infinite traces: Rules~\textsc{(5)}
and~\textsc{(6)} guarantee that any execution of a smart contract
terminates, as the gas consumed is limited to the amount of gas set in
the blockchain variable \code{GAS} at the beginning of the execution.
Therefore, an execution trace terminates either because it runs out of
gas, or the last state of the trace is of the form
$\tuple{\semempty,\semlocal_{n},\semstorage_{n},\semgasop_{n},
  \semgasmem_{n}}$, where $\semempty$ is the empty sequence of
activation records, $\semlocal_{n}$ and $\semstorage_{n}$ represent
the final mappings of the local variables and storage variables,
respectively, and $\semgasop_{n} + \semgasmem_{n}$ is the total gas
consumed in the execution of the program according to the cost
specified in~\cite{yellow}, as we will see in next section.



